Beyond Complete Shapes: A Benchmark for Quantitative Evaluation of 3D Shape Surface Matching Algorithms

Finding correspondences between 3D deformable shapes is an important and long-standing problem in geometry processing, computer vision, graphics, and beyond. While various shape matching datasets exist, they are mostly static or limited in size, restricting their adaptation to different problem settings, including both full and partial shape matching. In particular the existing partial shape matching datasets are small (fewer than 100 shapes) and thus unsuitable for data-hungry machine learning approaches. Moreover, the type of partiality present in existing datasets is often artificial and far from realistic. To address these limitations, we introduce a generic and flexible framework for the procedural generation of challenging full and partial shape matching datasets. Our framework allows the propagation of custom annotations across shapes, making it useful for various applications. By utilising our framework and manually creating cross-dataset correspondences between seven existing (complete geometry) shape matching datasets, we propose a new large benchmark BeCoS with a total of 2543 shapes. Based on this, we offer several challenging benchmark settings, covering both full and partial matching, for which we evaluate respective state-of-the-art methods as baselines.

==> tab/tab_all_datasets.tex <==
\begin{table}[ht]
\footnotesize
\centering
\begin{tabular}{@{}lccc@{}}
    \toprule
     \multirow{2}{*}{\textbf{Dataset}} & \textbf{\# Unique} & \textbf{Shape} & \textbf{Non}\\
     \textbf{} & \textbf{Shapes} & \textbf{Type} & \textbf{Isometry}\\
    \midrule
FAUST~\cite{bogo2014faust}                                                              & 100 & \Strichmaxerl & \xmark \\
SCAPE~\cite{anguelov2005scape}                                                          & 71  & \Strichmaxerl & \xmark \\
SMAL~\cite{Zuffi:CVPR:2017}                                          & 49 & \Cat & \cmark\\
DT4D Human~\cite{magnet2022smooth, li20214dcomplete}                 & 248 & \Strichmaxerl & (\cmark)\\
DT4D Animal~\cite{magnet2022smooth, li20214dcomplete}               & 1950 & \Cat & (\cmark)\\
TOSCA Human~\cite{bronstein2008numerical}                                               & 45 & \Strichmaxerl & \xmark\\
TOSCA Four-legged~\cite{bronstein2008numerical}                                         & 37 & \Cat & \xmark\\
KIDS~\cite{rodola2014dense}                                                             & 32    & \Strichmaxerl & \xmark\\
SHREC'20~\cite{dyke2020shrec}                                        & 11 & \Cat & \cmark\\
\midrule
\textbf{Ours}                                                                           & 2543 & \Strichmaxerl / \Cat & \cmark\\
\bottomrule
\end{tabular}
\caption{
\textbf{Overview of the data} that we use in our shape correspondence benchmark with their number of unique shapes, shape type (Humanoid \Strichmaxerl or Four-legged \Cat) and deformation class (Near-Isometric (\xmark) and Non-Isometric (\cmark)). We manually annotate shape correspondences across categories and datasets to increase the possible correspondence pairs significantly. \ve{move up}}
\label{tab:datasets}
\end{table}


==> vis/qualitative_full_full/qualitative_results_full_full.tex <==
\begin{figure*}[h!]
    \centering
    \begin{tabular}{@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}}
    \setlength{\tabcolsep}{0pt}  %
        
        \\
        
        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{SHREC'20 \\ $+$ DT4D}}}}} &
        \adjustbox{valign=m}{\includegraphics[height=0.07\textheight]{vis/qualitative_full_full/source_full_full_test_4.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.175\textwidth]{vis/qualitative_full_full/gt_full_full_test_4.png}
                \put(0, 45){\includegraphics[width=0.75cm]{vis/square_orange.png}}
            \end{overpic}   
        } &
        \adjustbox{valign=m}{\includegraphics[width=0.175\textwidth]{vis/qualitative_full_full/smooth_shells_full_full_test_4.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.173\textwidth]{vis/qualitative_full_full/geomfmaps_full_full_test_4.png}
                \put(65, 0){\includegraphics[width=0.75cm]{vis/circle_orange.png}}
            \end{overpic}   
        }
        
        &
        \adjustbox{valign=m}{\includegraphics[width=0.175\textwidth]{vis/qualitative_full_full/ulrssm_full_full_test_4.png}}  \\
        
        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{TOSCA \\ $+$ DT4D}}}}} &
        \adjustbox{valign=m}{\includegraphics[height=0.07\textheight]{vis/qualitative_full_full/source_full_full_test_32.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.173\textwidth]{vis/qualitative_full_full/gt_full_full_test_32.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.173\textwidth]{vis/qualitative_full_full/smooth_shells_full_full_test_32.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.173\textwidth]{vis/qualitative_full_full/geomfmaps_full_full_test_32.png}
                \put(72, 65){\includegraphics[width=0.75cm]{vis/circle_orange.png}}
            \end{overpic}   
        }
        
        &
        \adjustbox{valign=m}{\includegraphics[width=0.173\textwidth]{vis/qualitative_full_full/ulrssm_full_full_test_32.png}}  \\

        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{SHREC'20 \\ $+$ DT4D}}}}} &
        \adjustbox{valign=m}{\includegraphics[height=0.1\textheight]{vis/qualitative_full_full/source_full_full_test_68.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.075\textheight]{vis/qualitative_full_full/gt_full_full_test_68.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.075\textheight]{vis/qualitative_full_full/smooth_shells_full_full_test_68.png}
                \put(72, 45){\includegraphics[width=0.75cm]{vis/circle_orange.png}}
            \end{overpic}   
        }
        
        &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.075\textheight]{vis/qualitative_full_full/geomfmaps_full_full_test_68.png}
                \put(72, 45){\includegraphics[width=0.75cm]{vis/circle_orange.png}}
            \end{overpic}   
        }
        
        &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.075\textheight]{vis/qualitative_full_full/ulrssm_full_full_test_68.png}
                \put(72, 45){\includegraphics[width=0.75cm]{vis/circle_orange.png}}
            \end{overpic}   
        }
        
        \\
        & 
        Source &
        GT &
        Smooth Shells &
        GeomFMaps &
        ULRSSM  \\
    \end{tabular}
    \caption{\textbf{Cross-dataset and cross-category full-to-full shape matching results} visualized via colour transfer (red denotes unmatched parts).
    Our ground-truth correspondences include information about unmatchable parts (orange square). Existing methods have good performance overall. However, they do fail in some cases (orange circles).}
    \label{fig:F2F}
\end{figure*}


==> vis/qualitative_partial_full/qualitative_partial_full.tex <==
\begin{figure*}[h!]
    \centering
    \begin{tabular}{@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}}
    \setlength{\tabcolsep}{0pt}  % Set column separation to zero
        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{SHREC'20 \\ $+$ DT4D}}}}} &
        \adjustbox{valign=m}{\includegraphics[width=0.2\textwidth]{vis/qualitative_partial_full/source_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{vis/qualitative_partial_full/gt_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{vis/qualitative_partial_full/pfm_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{vis/qualitative_partial_full/dpfm_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{vis/qualitative_partial_full/ulrssm_partial_full_test_6.png}}\\
        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{FAUST \\ $+$ KIDS}}}}} &
        \adjustbox{valign=m}{\includegraphics[height=0.12\textheight]{vis/qualitative_partial_full/source_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.12\textheight]{vis/qualitative_partial_full/gt_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.12\textheight]{vis/qualitative_partial_full/pfm_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.12\textheight]{vis/qualitative_partial_full/dpfm_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.12\textheight]{vis/qualitative_partial_full/ulrssm_partial_full_test_26.png}} \\
        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{DT4D \\ $+$ TOSCA}}}}} &
        \adjustbox{valign=m}{\includegraphics[height=0.12\textheight]{vis/qualitative_partial_full/source_partial_full_test_27.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{vis/qualitative_partial_full/gt_partial_full_test_27.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{vis/qualitative_partial_full/pfm_partial_full_test_27.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{vis/qualitative_partial_full/dpfm_partial_full_test_27.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{vis/qualitative_partial_full/ulrssm_partial_full_test_27.png}}\\
         &
        Source &
        GT &
        PFM &
        DPFM &
        ULRSSM  \\
    \end{tabular}
    \caption{\textbf{Cross-dataset and cross-category partial-to-full shape matching results} visualized via colour transfer.
    Overall, all baselines have sub-optimal performance. Among them, DPFM (supervised method) shows the best results out of the three baselines. PFM and ULRSSM predict random correspondences between source and target shapes, notably visible on the cat's back and rhino's belly in the first and third rows, respectively.}
    \label{fig:P2F}
\end{figure*}

==> vis/qualitative_partial_partial/qualitative_partial_partial.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{tabular}{@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}}
    \setlength{\tabcolsep}{0pt}  %
        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{DT4D \\ $+$ DT4D}}}}} &
        \adjustbox{valign=m}{\includegraphics[height=0.08\textheight]{vis/qualitative_partial_partial/source_partial_partial_test_22.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.09\textheight]{vis/qualitative_partial_partial/gt_partial_partial_test_22.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.09\textheight]{vis/qualitative_partial_partial/dpfm_partial_partial_test_22.png}
                \put(0, 30){\includegraphics[width=0.75cm]{vis/circle.png}}
            \end{overpic}    
        } &
        \adjustbox{valign=m}{\includegraphics[height=0.09\textheight]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_22.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.09\textheight]{vis/qualitative_partial_partial/gc_ppsm_partial_partial_test_22.png}}  \\
        
        
        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{TOSCA \\ $+$ DT4D}}}}} &
        \adjustbox{valign=m}{\includegraphics[height=0.11\textheight]{vis/qualitative_partial_partial/source_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.08\textheight]{vis/qualitative_partial_partial/gt_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.08\textheight]{vis/qualitative_partial_partial/dpfm_partial_partial_test_42.png}
                \put(10, 60){\includegraphics[width=0.75cm]{vis/circle.png}}
            \end{overpic}    
        } &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.08\textheight]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_42.png}
                \put(10, 50){\includegraphics[width=0.9cm]{vis/square.png}}
            \end{overpic}   
        } &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.08\textheight]{vis/qualitative_partial_partial/gc_ppsm_partial_partial_test_42.png}
                \put(20, 50){\includegraphics[width=0.9cm]{vis/square.png}}
            \end{overpic}   
        } \\

        
        \adjustbox{valign=m}{\rotatedCentering{90}{\heightIQ}{\textbf{\small{\shortstack{KIDS \\ $+$ SCAPE}}}}} &
        \adjustbox{valign=m}{\includegraphics[height=0.11\textheight]{vis/qualitative_partial_partial/source_partial_partial_test_67.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.11\textheight]{vis/qualitative_partial_partial/gt_partial_partial_test_67.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.11\textheight]{vis/qualitative_partial_partial/dpfm_partial_partial_test_67.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.11\textheight]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_67.png}
                \put(0, 25){\includegraphics[width=0.9cm]{vis/square.png}}
            \end{overpic}   
        } &
        \adjustbox{valign=m}{\includegraphics[height=0.11\textheight]{vis/qualitative_partial_partial/gc_ppsm_partial_partial_test_67.png}} \\

         &
        Source &
        GT &
        DPFM &
        SM-COMB &
        GC-PPSM  \\
    \end{tabular}
    \caption{\textbf{Cross-dataset and cross-category partial-to-partial shape matching} results visualized via colour transfer (red denotes unmatched parts). All three baselines show sub-optimal performance. DPFM tends to predict random correspondences (blue circles).
    SM-COMB and GC-PPSM are unable to predict correspondences on large portions of the shapes (blue squares).
    }
    \label{fig:P2P}
\end{figure*}


==> vis/qualitative_results_all/qualitative_all.tex <==
\begin{figure}[!ht]
    \centering
    \begin{tabular}{@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}} \toprule
    \setlength{\tabcolsep}{0pt}  %
        
        \multirow{4}{*}[-3em]{\rotatebox[origin=c]{90}{\footnotesize{\textit{Full-to-Full (F2F)}}}} & 
        \scriptsize{Source} &
        \scriptsize{GT} &
        \scriptsize{GeomFMaps} &
        \scriptsize{ULRSSM} &
        \scriptsize{Smooth Shells}\\

        &
        \adjustbox{valign=m}{\includegraphics[height=0.04\textheight]{vis/qualitative_full_full/source_full_full_test_4_new.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.072\textwidth]{vis/qualitative_full_full/gt_full_full_test_4.png}
                \put(-3, 45){\includegraphics[width=0.45cm]{vis/green_sqaure.png}}
            \end{overpic}   
        } &
        \adjustbox{valign=m}{\includegraphics[width=0.072\textwidth]{vis/qualitative_full_full/geomfmaps_full_full_test_4.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.072\textwidth]{vis/qualitative_full_full/ulrssm_full_full_test_4.png}}  &
        \adjustbox{valign=m}{\includegraphics[width=0.072\textwidth]{vis/qualitative_full_full/smooth_shells_full_full_test_4.png}} \\

        
        &
        \adjustbox{valign=m}{\includegraphics[height=0.04\textheight]{vis/qualitative_full_full/source_full_full_test_32.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/gt_full_full_test_32.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/geomfmaps_full_full_test_32.png}} &        %
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.085\textwidth]{vis/qualitative_full_full/ulrssm_full_full_test_32.png}
                \put(0, 12){\includegraphics[width=0.4cm]{vis/blue_circle.png}}
            \end{overpic}   
        } 
        &
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/smooth_shells_full_full_test_32.png}}\\
        &
        \adjustbox{valign=m}{\includegraphics[height=0.06\textheight]{vis/qualitative_full_full/source_full_full_test_68.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.045\textheight]{vis/qualitative_full_full/gt_full_full_test_68.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.045\textheight]{vis/qualitative_full_full/geomfmaps_full_full_test_68.png}
                \put(78, 48){\includegraphics[width=0.4cm]{vis/blue_circle.png}}
            \end{overpic}   
        } &
        \adjustbox{valign=m}{\includegraphics[height=0.045\textheight]{vis/qualitative_full_full/ulrssm_full_full_test_68.png}}  &
        \adjustbox{valign=m}{\includegraphics[height=0.045\textheight]{vis/qualitative_full_full/smooth_shells_full_full_test_68.png}} \\



        \midrule
        \multirow{4}{*}[-2em]{\rotatebox[origin=c]{90}{\footnotesize{\textit{Partial-to-Full (P2F)}}}} & 
        \scriptsize{Source} &
        \scriptsize{GT} &
        \scriptsize{DPFM~\tiny{(\textit{Unsup})}} &
        \scriptsize{ULRSSM} &
        \scriptsize{PFM} \\

        &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/source_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/gt_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/dpfm_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/ulrssm_partial_full_test_6.png}} &
                \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/pfm_partial_full_test_6.png}}\\


        &
        \adjustbox{valign=m}{\includegraphics[height=0.06\textheight]{vis/qualitative_partial_full/source_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.07\textheight]{vis/qualitative_partial_full/gt_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.07\textheight]{vis/qualitative_partial_full/dpfm_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.07\textheight]{vis/qualitative_partial_full/ulrssm_partial_full_test_26.png}} &
                \adjustbox{valign=m}{\includegraphics[height=0.07\textheight]{vis/qualitative_partial_full/pfm_partial_full_test_26.png}}\\

        
        &
        \adjustbox{valign=m}{\includegraphics[height=0.06\textheight]{vis/qualitative_partial_full/source_partial_full_test_27.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.075\textwidth]{vis/qualitative_partial_full/gt_partial_full_test_27.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.075\textwidth]{vis/qualitative_partial_full/dpfm_partial_full_test_27.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.075\textwidth]{vis/qualitative_partial_full/ulrssm_partial_full_test_27.png}} &
                \adjustbox{valign=m}{\includegraphics[width=0.075\textwidth]{vis/qualitative_partial_full/pfm_partial_full_test_27.png}}\\

    
        \midrule

        \multirow{4}{*}[-2.5em]{\rotatebox[origin=c]{90}{\footnotesize{\textit{Partial-to-Partial (P2P)}}}} & 
        \scriptsize{Source} &
        \scriptsize{GT} &
        \scriptsize{DPFM~\tiny{\textit{(Sup)}}} &
        \scriptsize{SM-COMB} &
        \scriptsize{GC-PPSM} \\

        &
        \adjustbox{valign=m}{\includegraphics[height=0.05\textheight]{vis/qualitative_partial_partial/source_partial_partial_test_22.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.06\textheight]{vis/qualitative_partial_partial/gt_partial_partial_test_22.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[height=0.06\textheight]{vis/qualitative_partial_partial/dpfm_partial_partial_test_22.png}
                \put(0, 30){\includegraphics[width=0.4cm]{vis/blue_circle.png}}
            \end{overpic}    
        } &
        \adjustbox{valign=m}{\includegraphics[height=0.06\textheight]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_22.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.06\textheight]{vis/qualitative_partial_partial/vik_partial_partial_test_22.png}}  \\

        
        &
        \adjustbox{valign=m}{\includegraphics[height=0.06\textheight]{vis/qualitative_partial_partial/source_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.05\textheight]{vis/qualitative_partial_partial/gt_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.05\textheight]{vis/qualitative_partial_partial/dpfm_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.05\textheight]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.05\textheight]{vis/qualitative_partial_partial/vik_partial_partial_test_42.png}} \\

        
        &
        \adjustbox{valign=m}{\includegraphics[height=0.08\textheight]{vis/qualitative_partial_partial/source_partial_partial_test_67.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.08\textheight]{vis/qualitative_partial_partial/gt_partial_partial_test_67.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.08\textheight]{vis/qualitative_partial_partial/dpfm_partial_partial_test_67.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.08\textheight]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_67.png}} &
        \adjustbox{valign=m}{\includegraphics[height=0.08\textheight]{vis/qualitative_partial_partial/vik_partial_partial_test_67.png}} \\
        
            
        \bottomrule

    \end{tabular}
    \caption{\textbf{Cross-dataset and cross-category shape matching} results visualized via colour transfer (red denotes unmatched parts). All baselines show sub-optimal performance on all three settings as shown with the blue circles. The green square shows the semantically unmatchable parts between the source and target mesh.}
    \label{fig:all_qualitative_results}
\end{figure}


==> vis/qualitative_results_all/qualitative_all_double_column_row_wise.tex <==
\begin{figure*}[!ht]
    \centering
    \setlength{\tabcolsep}{3pt} 
    \begin{tabular}{cc@{}c@{}c?cc@{}c@{}c?cc@{}c@{}c@{}}
        
        \multicolumn{4} {c?} {\normalsize{\textit{\textbf{Full-to-Full (F2F)}}}} &
        \multicolumn{4} {c?} {\normalsize{\textit{\textbf{Partial-to-Full (P2F)}}}} & 
        \multicolumn{4} {c} {\normalsize{\textit{\textbf{Partial-to-Partial (P2P)}}}} \\ 

        \rotatebox[origin=c]{90}{\small{Source}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.12\textwidth]{vis/qualitative_full_full/source_full_full_test_4_new.png}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.1\textwidth]{vis/qualitative_full_full/source_full_full_test_32.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.07\textwidth]{vis/qualitative_full_full/source_full_full_test_68.png}} &

        \rotatebox[origin=c]{90}{\small{Source}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.12\textwidth]{vis/qualitative_partial_full/source_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.04\textwidth]{vis/qualitative_partial_full/source_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.1\textwidth]{vis/qualitative_partial_full/source_partial_full_test_27.png}} &

        \rotatebox[origin=c]{90}{\small{Source}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.1\textwidth]{vis/qualitative_partial_partial/source_partial_partial_test_22.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.1\textwidth]{vis/qualitative_partial_partial/source_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.04\textwidth]{vis/qualitative_partial_partial/source_partial_partial_test_67.png}} \\


        \rotatebox[origin=c]{90}{\small{GT}} & 
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.085\textwidth]{vis/qualitative_full_full/gt_full_full_test_4.png}
                \put(-3, 45){\includegraphics[width=0.45cm]{vis/green_sqaure.png}}
            \end{overpic}   
        } &
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/gt_full_full_test_32.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.1\textwidth]{vis/qualitative_full_full/gt_full_full_test_68.png}} &

        \rotatebox[origin=c]{90}{\small{GT}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.12\textwidth]{vis/qualitative_partial_full/gt_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.07\textwidth]{vis/qualitative_partial_full/gt_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/gt_partial_full_test_27.png}} &

        \rotatebox[origin=c]{90}{\small{GT}} & 
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.08\textwidth]{vis/qualitative_partial_partial/dpfm_partial_partial_test_22.png}
                \put(0, 30){\includegraphics[width=0.4cm]{vis/blue_circle.png}}
            \end{overpic}    
        } &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_partial/gt_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.05\textwidth]{vis/qualitative_partial_partial/gt_partial_partial_test_67.png}} \\


        \rotatebox[origin=c]{90}{\small{GeomFMaps}} &
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/geomfmaps_full_full_test_4.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/geomfmaps_full_full_test_32.png}} &
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.1\textwidth]{vis/qualitative_full_full/geomfmaps_full_full_test_68.png}
                \put(82, 50){\includegraphics[width=0.4cm]{vis/blue_circle.png}}
            \end{overpic}   
        } &

        \rotatebox[origin=c]{90}{\small{DPFM}~\footnotesize{(\textit{Unsup})}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.12\textwidth]{vis/qualitative_partial_full/dpfm_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.07\textwidth]{vis/qualitative_partial_full/dpfm_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/dpfm_partial_full_test_27.png}} &

        \rotatebox[origin=c]{90}{\small{DPFM}~\footnotesize{(\textit{Sup})}} & 
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.08\textwidth]{vis/qualitative_partial_partial/dpfm_partial_partial_test_22.png}
                \put(0, 30){\includegraphics[width=0.4cm]{vis/blue_circle.png}}
            \end{overpic}    
        } &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_partial/dpfm_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.05\textwidth]{vis/qualitative_partial_partial/dpfm_partial_partial_test_67.png}} \\


        \rotatebox[origin=c]{90}{\small{ULRSSM}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/ulrssm_full_full_test_4.png}}  &
        \adjustbox{valign=m}{
            \begin{overpic}[width=0.085\textwidth]{vis/qualitative_full_full/ulrssm_full_full_test_32.png}
                \put(0, 12){\includegraphics[width=0.4cm]{vis/blue_circle.png}}
            \end{overpic}   
        } &
        \adjustbox{valign=m}{\includegraphics[width=0.1\textwidth]{vis/qualitative_full_full/ulrssm_full_full_test_68.png}}  &


        \rotatebox[origin=c]{90}{\small{ULRSSM}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.12\textwidth]{vis/qualitative_partial_full/ulrssm_partial_full_test_6.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.07\textwidth]{vis/qualitative_partial_full/ulrssm_partial_full_test_26.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/ulrssm_partial_full_test_27.png}} &

        \rotatebox[origin=c]{90}{\small{SM-COMB}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_22.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_42.png}} &
        \adjustbox{valign=m}{\includegraphics[width=0.05\textwidth]{vis/qualitative_partial_partial/sm_comb_partial_partial_test_67.png}} \\


        \rotatebox[origin=c]{90}{\small{Smooth Shells}} &
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/smooth_shells_full_full_test_4.png}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.085\textwidth]{vis/qualitative_full_full/smooth_shells_full_full_test_32.png}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.1\textwidth]{vis/qualitative_full_full/smooth_shells_full_full_test_68.png}} & 

        \rotatebox[origin=c]{90}{\small{PFM}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.12\textwidth]{vis/qualitative_partial_full/pfm_partial_full_test_6.png}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.07\textwidth]{vis/qualitative_partial_full/pfm_partial_full_test_26.png}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_full/pfm_partial_full_test_27.png}} & 

        \rotatebox[origin=c]{90}{\small{GC-PPSM}} &
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_partial/vik_partial_partial_test_22.png}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.08\textwidth]{vis/qualitative_partial_partial/vik_partial_partial_test_42.png}} & 
        \adjustbox{valign=m}{\includegraphics[width=0.05\textwidth]{vis/qualitative_partial_partial/vik_partial_partial_test_67.png}} \\
        
        

    \end{tabular}
    \caption{\textbf{Cross-dataset and cross-category shape matching} results visualized via colour transfer (red denotes unmatched parts). All baselines show sub-optimal performance on all three settings as shown with the blue circles. The green square shows the semantically unmatchable parts between the source and target mesh.}
    \label{fig:all_qualitative_results}
\end{figure*}

